Turbocharge Speech Understanding with Pilot Inference

Modern speech understanding (SU) runs a sophisticated pipeline: ingesting streaming voice input, the pipeline executes encoder-decoder based deep neural networks repeatedly; by doing so, the pipeline generates tentative outputs (called hypotheses), and periodically scores the hypotheses. This paper sets to accelerate SU on resource-constrained edge devices. It takes a hybrid approach: to speed up on-device execution; to offload inputs that are beyond the device's capacity. While the approach is well-known, we address SU's unique challenges with novel techniques: (1) late contextualization, which executes a model's attentive encoder in parallel to the input ingestion; (2) pilot inference, which mitigates the SU pipeline's temporal load imbalance; (3) autoregression offramps, which evaluate offloading decisions based on pilot inferences and hypotheses. Our techniques are compatible with existing speech models, pipelines, and frameworks; they can be applied independently or in combination. Our prototype, called PASU, is tested on Arm platforms with 6 - 8 cores: it delivers SOTA accuracy; it reduces the end-to-end latency by 2x and reduces the offloading needs by 2x.

==> conclusion.tex <==
\section{Conclusion}


==> fig-models.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.48\textwidth]{./figs/models}
	%	\vspace{-2em}
	\caption{Compared to popular encoder-decoder SU models (left), our model (right) shifts much of the encoding computation to bottom layers, allowing them to be executed in a streaming fashion during ingestion.
 XXX show segment by segment input... XXX 
	}
	\label{fig:mo}
	%	\vspace{-5mm}
\end{figure}

==> fig-tctc.tex <==
\begin{figure}[t!]
	\centering
	\includegraphics[width=0.48\textwidth]{./figs/tctc}
	%	\vspace{-2em}
	% \caption{The offloading break down of selective offloading and sampling offloading. Selective offloading can help largely reduce the offloading data count by preventing offload non-target data}
	%\caption{Three decoding speedup techniques all contributes to decoding speedup, sum up to 1.5x speedup. LP: length prediction, BR: Beam reduce, CS: CTC prefix scoring speedup}
	%\label{fig:}
	\caption{Truncate CTC algorithm in Online hybrid CTC/Attention. Base on the peaky CTC assumption, the algorithm discard part of the computation on later time frame after the CTC peak}
	\label{fig：tctc}
	%	\vspace{-5mm}
\end{figure}

==> figs/tmp-pdfcrop-12212.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{706C6174666F726D73706563732E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}
\page 1 [89 676 460 721]
\csname @@end\endcsname
\end


==> figs/tmp-pdfcrop-33744.tex <==
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
\def\pdffilehex{6374636C6561702E7064662E756E63726F70}
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
\pdfcompresslevel=9  \pdfoutput=1 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1#2{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1=1 %
     \ifnum#2<5
       \pdfobjcompresslevel=0 %
     \else
       \pdfobjcompresslevel=2 %
     \fi
   \fi 
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#2\relax
    }%
  }{%
    \pdfminorversion=#2\relax
    \IfUndefined{pdfmajorversion}{%
      \ifnum#2=0 \pdfminorversion=5\fi}
      {\pdfmajorversion=#1\relax}%
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
\setpdfversion{1}{7}


==> intro__Felix_s_conflicted_copy_2024-03-05_.tex <==
% !TeX root = main.tex

\section{Introduction}
\label{sec:intro}


Speech is a pervasive user interface for embedded devices. 
% It is in particular useful to small embedded/IoT devices where hands free interactions are desirable. 
At its core are two speech understanding (SU) tasks: 
automatic speech recognition (ASR), transcribing voice to a sentence~\cite{yu2016automatic};
spoken language understanding (SLU), mapping voice to a structured intent, such as 
\code{\{scenario: Calendar, action: Create\_entry\}}~\cite{de2007spoken}.


\xzlNote{below: connect to figure 1}

\paragraph{Modern SU: autoregression with beam search}
Modern SU runs a deep, encoder-decoder model \cite{Jan2015NIPS} as shown in \autoref{fig:intro}(a). 
Ingesting an utterance waveform, the model comprises a neural encoder and a neural decoder, 
generating a sequence of tokens, i.e. words or sub-words. 
This generation process is \textit{autoregressive}: 
to produce a token, the decoder takes as the input all the latent units from the encoder, 
as well the output tokens it produces so far. 
% the generation of the next token is conditioned on the previous output tokens and runs these layers again. 
To cope with noisy utterances, SU runs multiple decoding processes in parallel, 
each generating a candidate output sequence (called a hypothesis). 
SU picks the best sequence as the final output. 
Thanks to the encoder/decoder wrapped in beam search, 
modern SU can understand natural utterances (e.g. ``I need to turn on light in bedroom '')~\cite{slurp_dataset} beyond simple ones (e.g. ``light on'').
This paper focuses on encoder-decoder SU models. 

Deep SU models are resource-hungry. 
The ones with satisfactory accuracy often require GBs of memory and tens of GFLOPs per input second~\cite{arora2022two}; 
even after compression to fit in embedded devices, the resultant models can take more than 10 seconds to process an input of a few seconds. 
Facing the constraints, many embedded devices chose to 
offload \textit{all} voice inputs to the cloud~\cite{microsoft_azure_speech}, 
which, however, raises concerns on high cloud cost~\cite{qualcomm2023hybridcost, qualcomm2023futurehybridai, microsoft2023azurehybridbenefit}, privacy~\cite{saade2019spoken}, latency~\cite{maheshwari2018latency}, and service availability. 
\input{fig-intro}
\paragraph{Problem \& approach}
This paper sets to accelerate deep SU on resource-constrained embedded devices\footnote{Referred to as ``devices'' for simplicity, will be defined in \sect{motiv}}.
\xzlNote{simplify below}
It presents an on-device SU engine that integrates a local execution path and an offloading path; 
the local path optimized to reduce on-device latencies and the offloading selectively offloads the inputs beyond the device's capacity, hence ensuring the overall accuracy. 
%Both aspects are vital; 
% pairing the on-device model with large cloud model but offers gold accuracy. 
%\input{fig-intro}
While the local/offloading approach is reminiscent of many ML systems, e.g. for vision and NLP~\cite{shakarami2020survey,yao2020deep,lv2022walle}, our design specifically addresses unique challenges from speech. 
This is shown in \autoref{fig:intro}(b). 

\subsection{The local execution path}

\xzlNote{simplify...}
\paragraph{Challenge: temporal load imbalance}
We identify a key SU inefficiency: 
poor resource utilization during the ingestion time. 
% the model under utilizes computational resource during the ingestion time. 
While a typical utterance spans at least several seconds, 
the compute is mostly idle during the ingestion period, 
because most of an encoder-decoder model is to be executed over a complete input, thanks to its all-to-all attention. \xzlNote{connect to fifgure 1}
Yet, as soon as the ingestion completes, 
a surge of workload --- encoding and then decoding -- emerges, 
for which long delays are directly perceived by the user. 

Naively processing truncated (i.e. yet to complete) utterances \textit{during} ingestion would result in 
significant errors, as SU models were trained on, and therefore expect, complete utterances. 
% it do not expect an utterance to be trunacanted and thereore produces errorneous output. 
While some SU models are designed to process streaming inputs, 
they often make significant compromise on accuracy~\cite{kuo2020interspeech,li2020comparisone2emodel}, as will be discussed in \sect{related}.

In summary, the device needs to utilize ingestion-time resources to accelerate the expensive processing that can only start after the ingestion. \xzlNote{reword}

%\paragraph{Design: streaming encoding with pilot inference}
\paragraph{Our design}
%
Our first technique, called \textit{late contextualization}, refactors an SU model
so that most of encoding layers can execute in parallel to ingestion. 
Rather than computing all-to-all attention at each encoding layer, 
we make the bottom layers (closer to the input) compute only convolution, and the few top layers compute attention. \xzlNote{downplay this}

Our second techique is called \textit{pilot inference}: 
during ingestion, SU periodically encodes and decodes the incomplete input accumulated so far. 
%The output cannot be materialized: 
%since the input is still incomplete, the output sequence is likely to contain substantial incorrect tokens near its end where the input is cutoff
%(e.g. ... ). 
% However, the beam search trace in pilot decoding can accelerate the full decoding, i.e. on the complete input after the ingestion: 
% However, the beam search trace in pilot decoding can accelerate the full decoding that consumes the complete input: 
% at low cost, the full decoding simply verify if the output token from pilot decoding are still valid, and only starts expensive beam search in case 
As mentioned above, inference on a truncated input will result in substantial errors, particularly near the output sequence's end. 
Yet, our key insight is that the the \xzlNote{piolot..} inference's \textit{intermediate state} can assist the subsequent full inference (i.e. the one executed over the complete input). 
The assistance comes in multiple ways: 
(1) beam collapse: 
the full inference only needs to verify its beam search path against the path in the pilot inference, and only falls back to full beam search in case of path divergence;
(2) early termination: 
extrapolating the output length of pilot inference, the full inference predicts the final output length and prunes astray search paths;
(3) CTC leap: approximating the CTC prefix scoring~\cite{watanane2017hybridctc} with the scores already computed in pilot inferences. 

\xzlNote{move here}
it does so by scoring all hypotheses with attention and CTC (\ctc{})~\cite{watanane2017hybridctc}. 


%A nice property of pilot inferences is being incremental: 
Pilot inferences are cheap: 
being incremental, the $(i+1)$-th inference instance reuses of the state from the $i$-th instance, 
in the same way as the full inference reuses the last pilot inference instance. 
In this way, the total cost of pilot inference is amortized over the duration of ingestion, and scales gracefully with the input length. 

Pilot inference (PI) is related to recent speculative execution for language models~\cite{kim2023speculative} with a key difference: 
while the later optimizes inference on \textit{complete} inputs, 
PI processes successive \textit{incomplete} inputs, 
entailing different challenges and techniques. 
\sect{related} presents a detailed comparison. 

\subsection{The offloading path}

\paragraph{Challenge: Offramps for autoregression}
%
The common offloading paradigm works as follows.
To decide whether to offload an input $x$, 
the device assesses how likely the on-device inference yields a sufficiently accurate answer.  
Often, such an assessment of \textit{confidence} is based on shallow processing of $x$, 
which is referred to as \textit{offramps} in prior work.
% leaving time for the subsequent offloading or local inference. 
Existing offramp designs typically evaluates confidence as an ML model's prediction entropy~\cite{NEURIPS2020_d4dd111a,xin-etal-2020-deebert}. 
% which is derived from thge model's intermediate state or final output. 
For SU however, existing offramps mismatch in two ways. 

% Speech is different on multiple key aspects. 
First is the \textit{confidence measure}. 
Unlike a classification task which evaluate a model's layers sequentially,  
SU's output generation is both concurrent and iterative:  
it produces multiple hypotheses of probabilistic tokens; 
to produce each token it evaluates all the decoder layers. 
To complicate the issue, 
one hypothesis often comprises tokens that have drastically different probabilities.
% As voice inputs are often noisy, low probability tokens are not uncommon even in a high confidence output sequence. 
It was unclear how to derive one confidence score out of such a generation process. 

Second is \textit{timing}. 
Given an input, offramp represents a one-shot decision that can be taken at various times throughout the SU pipeline shown in \autoref{fig:intro}. 
% during ingestion, after ingestion but somewhere in decoding, or after decoding. 
% once offloaded, the cloud cost is incurred and the input data is revealed. 
While a deferred decision would have more input information for measuring the model confidence, 
it also incurs substantial on-device delays. 
% should the offramp eventually decide to offload. 
% it also misses opportunities for early exiting to the cloud
The timing therefore hinges on tradeoffs between an offramp's selectivity and overhead. 

\paragraph{Our design}
%
The device evaluates its offloading decision as soon as it finishes ingestion, 
based on the perplexity score \cite{Jelinek1977PerplexityaMO} of the last pilot inference (LPI). 
Doing so strikes a sweet-spot: % between the offramp's selectivity and overhead: 
(1) as the discrepancy between the LPI and the full inference is small, 
their perplexity scores are also similar; 
(2) the device does not need to hold off the offloading decision until the slow full inference. 
% in case of a ``no offlaoding'' decision, the device can proceed to full decoding without any delay. 
% Note that ingestion completion is the earliest moment the device should offload: 
Note that offloading \textit{before} the ingestion completes does not reduce the offloading delay. 
As an input utterance is as small as tens of KB, 
%the upload is bound by network latency under typical network conditions; 
the upload is typically bound by network latency; 
another network round trip is nevertheless needed. 

%To assess the confidence, we demonstrate that based on decoding outcome is better. 
%We show that prior methods, e.g. confidence estimated from encoding layers, results in inferior decisions. 
%The key is to model the whole sequence rather than probabilities of individual tokens,
%We explore a variety of sequence modeling techniques (lightweight LSTM, 1D-CNN) and find perplexity score as a sweet-spot trade-off between complexity and accuracy. 

\subsection{Results and contributions}

%\paragraph{Results}
We implement a system called \sys{} (Pilot-Aid SU), 
atop two embedded platforms with 6 and 8 Arm64 cores respectively. 
We test \sys{} on SLURP~\cite{slurp_dataset}, a challenging speech benchmark comprising 102 hours of speech. 
On both ASR and SLU tasks, \sys{} delivers strong accuracies with end-to-end latencies as low as 100s of ms. 
\sys{}'s on-device execution incurs 2x lower latency as
compared to popular, efficiency-optimized models running on device \hl{with energy saving or little energy consumption overhead}. 
Combining local execution with offloading, \sys{}'s hybrid execution offers much higher accuracy than on-device models at similar or lower latency; 
the hybrid execution offers close-to-gold accuracy (only 1\% lower than SOTA), while requiring 47\% -- 53\% less offloading than offloading all the inputs. 


\begin{comment}
We implement \sys{} atop ESPnet \cite{watanabe2018espnet} and demonstrate it on mobile CPU and GPU of three embedded platforms. On two major SU tasks: ASR and SLU, \sys{} meets different target accuracy QoS while achieve state of the art low average RTF. We compare \sys{} against competitive baselines mentioned in previous works \cite{conformer-2020} \cite{peng2022branchformer} \cite{zhang2020transformer} as illustrated in Figure 1. Compared to local processing, \sys{} reaches a higher WER / IC with the same average RTF. Compared to cloud processing, \sys{} reaches same high WER / IC with x\% RTF reduction. Compared to the existing selective offload methods, with different target accuracy QoS, \sys{} shows y\% to z\% RTF reduction in average.
\end{comment}

%\paragraph{Contributions}
Towards deep SU on embedded devices, we contribute:

\begin{myitemize}
\item An encoder-decoder architecture (convolution on bottom layers; attention on top layers), which enable late contextualization and let most of the encoding computation finished during the ingestion%which suits early offloading on streaming (partial) inputs.
%\xzlNote{REWRITE THIS}

\item Pilot inference, a new techinque to exploit under-utilized resources during ingestion. 
% Note that pilot decoding, as a generic optimization technique, can be applied to other models without modifying their architectures. 

\item An offramp design that assesses model confidence in generative, autoregressive output. 
This is the first mechanism for offloading generative tasks, to the best of our knowledge. 
\end{myitemize}
	
We will make our model and code publicly available.	

%\xzlNote{highlight: two techinques applied indep, and in combination... both have benefiits}





 




==> recycle_buffer/detail.tex <==
% !TeX root = main.tex

\section{\sys{}: Streaming SLU Processing}
In this section, we provide a detailed explanation of how the major components of \sys{} are designed.

\subsection{Late contextualization and corresponding model design}

We design / co-trained \& deployed an encoder-decoder architecture based model that have customized design on both encoder and decoder to accommodate the streaming and full length data processing. 

Encoder design:
\sys{} adopt a late contextualization encoder design. The bottom layers only contains convolution, allows the model to process the streaming data. The top layers only contains transformer based all-to-all attention computation that exploit the contextual information for full length data processing. During the data processing, the bottom layers processing result of partial data will be cached, and reused for full length processing to avoid re-calculation.

Decoder design:
\sys{} provides two different decoder design for pilot decoding and full length inference. The pilot decoding requires low RTF to reach high granularity, thus need cheaper decoder and beam search design. \sys{} provide 1 layer transformer decoder for pilot decoding, also limit the beam search length within 15 tokens. For full length decoding, to reach a better influence accuracy, \sys{} provide 1 layers transformer decoder, higher beam size and beam search token limit.

\subsection{Pilot decoding and full decoding speedup} 

We design an offramp that consist decoder and decoding tracker (tree structured data based lstm) to help with the data inspection and confidence estimation. During the data ingestion, the 

\subsection{Selective offloading}


\xzlNote{moved here, to merge}

\textbf{why use RNN to model the output confidence?}
The intuition is that the consistency of hypotheses rankings, etc. 
For example, low-probability tokens, if occur in sequence, 
often imply that the model lacks confidence in the semantic correctness for a whole output span; 
% often imply that a span in the output has flawed structure or semantics; 
by contrast, if such tokens are just dispersed, it could be due to acoustic noise and the output is still mostly correct. 
Another example, a hypothesis ranked at the top at every decoding step shows higher confidence 
than a hypothesis with rankings fluctuates across decoding steps. 
While the rules can be difficult to define manually, we take a learning approach: 
% To model the dynamics and map it to confidence, 
we construct a lightweight BiLSTM (RNN?) model that predicts the SU accuracy based on the sequence of beam search features (\xzlNote{vague?})
The predicted accuracy serves as the basis of offloading decisions.	


 \subsection{Confidence prediction with beam search history}

 We design a scheduler, which can pre-profile the device and decide the partial granularities of partial decoding. Another important work of it is to decide which partial decoding result to use,  
 

==> recycle_buffer/eval__Felix_Lin_s_conflicted_copy_2023-09-19_.tex <==
% !TeX root = main.tex


\section{Evaluation}
\label{sec:eval}
%We evaluate \sys{} to address different aspects of the streaming SLU processing system:
We answer a few question through the evaluation process:
\begin{myitemize}
    \item Can \sys{} reduce the latency with compatible accuracy?
    \item How much do different key designs count for the benefits we see?
    \item How does several system parameters (hardware specification, network condition) affect the system?
\end{myitemize}
\xzlNote{to revisit after the whole eval is written}

\subsection{Methodology}
\paragraph{Test platform}
As shown in Table~\ref{tab:platforms}, we test our device runtime 
on two embedded boards: 
board 1 with an efficiency-oriented processor, 
board 2 with a performance-oriented processor. 
Note that although our device runtime runs on CPUs, 
the idea of \sys{} applies to GPUs. 


\begin{comment}
with different CPU specifications. The board 1 have relatively low performance CPU, represent the common embedded devices. The board 2, on the other hand, have more capable CPU. Note that although in the evaluation part we only conduct experiments on CPU boards, \sys{} should also work with GPU and shows similar benefits.
\end{comment}

%\xzlNote{cloud...} %\xzlNote{How is the cloud latency measured...}
We estimate the cloud offloading delays from real-world ML serving. 
To do so, we develop a test harness: 
running on an x86 desktop, it sends each input waveform to the Azure speech service \xzlNote{cite} and records wall clock time. 
The test was running from the US east coast and requests to use east coast datacenters. 
For each input, we repeat the test on enterprise WiFi (bandwidth in 100s of MB and RTT in ms) and on 5G cellular networks, and use the average delay. 
Note that we do not use the outcome of Azure speech for accuracy evaluation, because we often find its accuracy inferior to the SOTA model (XXX) used by us. 

\begin{comment}
We choose speech API provided by Microsoft Azure as the cloud baseline. The cloud latency of each audio is measured by uploading it through the Azure speech transcribing API under school WIFI and 5G hot spot, and we measure the time between uploading and result comes out. This measurement is solely for latency measurement. We do not rely on the accuracy of the Azure service but instead use the state-of-the-art model accuracy as the benchmark for cloud processing accuracy.
\end{comment}
    
\input{tab-platforms}

\paragraph{Dataset and model training}
%We trained models in our system on the SLURP dataset, run all the baselines and our system on the same dataset and inspect the metrics we mentioned above.
We run our experiments on the SLURP dataset comprising 101.5 hours of speech \xzlNote{cite}, as summarized in \xzlNote{Table XXX}. 
SLURP is widely considered challenging: 
unlike many datasets of short commands (e.g. ``light on''), 
SLURP's utterances are more complex and closer to daily human speech
(e.g. ``\xzlNote{.....}''). 
Of all 141530 utterances, we use 119880 (85\%) for training and the rest for test, 
from which accuracy and latency are reported. 


\begin{comment}
Our experiments are based on the SLURP dataset, a renowned SLU corpus. This dataset comprises 141530 audio files from 211 speakers, totaling 101.5 hours. The dataset consists of short command utterances with an average length of ~2.6s. All the data is transcribted and labeled with 69 different intents. Model training is conducted using the training set that contains 119880 data points. Accuracy and Latency measurement is on the test set with 8211 data points, length ranging from 2.2s to 6.2s.
\end{comment}


%Total: 13K, we picked: 8K
%(\textbf{could be a problem}...)

\paragraph{Metrics}
\underline{Accuracy:}
We follow the common practice. 
For ASR, we report word error rate (WER). 
WER is the discrepancy between the model output and the gold (ground truth?) transcript, 
 defined as count of errors (substitutions, deletions, insertions) normalized by the sentence length.  
 For SLU, we report the intent classification accuracy. %\wrxNote{Redundent: In SLURP dataset, every data entry has a intent corresponding to scenario plus action. There are 69 different intents in the SLURP dataset.}

\underline{Latency:}
(1) We report user-perceive latency: 
the elapsed time from a user completing her utterance to our system emitting the complete SU result. This metric is also used by prior work \xzlNote{cite}. 
(2) We further report real time factor (RTF): 
the user-perceived latency normalized by the input utterance's duration. 


\begin{comment}
 the absolute latency of the system (wall clock...) as the time between the finish of the utterance speaking and the completion of the ASR result generation. This is the latency in the real world using case. Besides absolute latency, we also adopt real time factor (RTF), which equals to absolute latency (or system elapse time) normalized by corresponding speech duration, as a normalized latency metric.
%what knobs we tune? --- threshold. (need to justify how to tune this)
%compare the resultant delays... (user perceived)
\end{comment}

\paragraph{Baselines}
We compare our system with several designed baselines.
\begin{myitemize}
    \item \textit{All local}: The system processes all the data on the local model. It choose the best local model setting with compatible model size. We selects a few popular model structures like conformer, branchformer, CNN-RNNT, modify their hyperparameters to let them have the similar model size.

    \item \textit{All cloud}: The system blindly offloads all the data to the cloud side. We adopted a 2 pass end-to-end SLU model proposed in \wrxNote{cite}. The model includes one conformer based encoder, one conformer based deliberation encoder, two transformer based decoders for the first and the second pass, and a pretrained BERT language model.
    
    %\item \textit{Random offload}: The system randomly offloads data with certain probability to meet the accuracy requirement. \xzlNote{needed?}
    
    %\item \textit{LC offload}: The system adopts a linear classifier to predict the local WER/IC and decide whether offload or not.
    %\item \textit{PS offload}: The system offloads data base on its local perplexing score in decoding process.
    \item \textit{Ours}: In \sys{}, there are a customized late contextualized local model, the selective offloading offramp and the pilot decoding orchestrated together. 
\end{myitemize}

\underline{Methods}
We compare the latency of our system and baselines with the same set of target accuracy. We first measure the latency and accuracy of local and cloud baselines. Then we define a series of accuracy target between local baseline accuracy and cloud accuracy. By tuning the confidence threshold, we configure our system to meet the accuracy target, measure and compare the latency with baseline / previous methods.

\input{fig-e2e}

\subsection{End-to-End results}


\paragraph{Overall latency and accuracy}
\sys{} achieve latency as low as xxx / xxx ms with compatible \xzlNote{comparable} accuracy. (WER, IC). Among all the accuracy targets, \sys{} consistently achieves the lowest overall latency with 30\%-50\% latency reduction compare to baselines as demonstrated in Figure~\ref{fig:eval:e2e}.  

%\xzlNote{be brief, or delete}
%The overall benefits come from two aspects of innovation in offload pass (which focus on local-cloud collaboration) and local pass (which focus on local process speed up).

\xzlNote{vs cloud}
Compare to the \textit{All cloud} baseline, \sys{} reduces the overall latency by as much as 30\% with less than 0.25 intent classification accuracy decrease. This efficiency arises from \sys{} meticulously analyzing data during local processing and making selective decisions about data offloading to the cloud in the offloading pass.

\xzlNote{vs all local}
In comparison to the \textit{All local} baseline, our system achieves a 50\% runtime acceleration while maintaining the same accuracy target. When setting the latency target to match local processing, our system enhances performance with a 6\% reduction in WER and a 2.5\% improvement in IC. This is due to \sys{} conducting pilot decoding during ingestion, which accelerates the local decoding process.



\xzlNote{Utilization and efficiency ... two separate things. We probably should focus on the former. But needed? -- can wait}
\paragraph{Computational resource efficiency}
We evaluate computational resource efficiency on local processing. %Figure~\ref{fig:eval:resource}
Experiments show the detailed GPU utilization for an audio data in average for baseline (top) and ours (bottom). In general, our system can finish the decoding in a shorter time period. During the ingestion time, the baseline conformer model do nothing but wait. 
Our system periodically conduct pilot decoding bases on partial data, take better usage of the idle resources. After ingestion time, the baseline model starts the encoding-decoding process, take relatively long time to finish. Our system only need to do the transformer part encoding, save the encoding time. Decoding time is also much shorter, with the help of our adaptive beam size reduction method.

\subsection{Efficacy of our local execution path}


%\xzlNote{Figure 2 must be referenenced and discussed}
%\xzlNote{In particular the RNN-T baseline...}

The delay of the local processing can be divided into two parts: encoding and decoding. 


%\xzlNote{Since table 2 focuses on on-device model structure... it might be a bit weird to include our WER/IC here. how about: maybe show conformer/branchformer/rnn-t WER/IC in Fig 1, as local baselines?}

%\xzlNote{Table 2: consider a column graph?}

\input{tab-models}
%\input{fig-models}
\input{tab-models2}

%\paragraph{local path: Late contextualization model design}
\paragraph{Encoding speedup}

\textbf{--- BELOW --- }
Our encoder design finds a sweet spot between speed (from streaming processing) and accuracy (from contextualization). 

Compared to full attention encoders (Conformer and Branchformers), our encoding latency is much lower by 0.07 - 0.1 RTF. This is because we locate 3 attention layers at the end part (top part) of the encoder. This late contextualization technique help significantly reduce the non-streaming flops in the encoder. Compare to the baseline attention based models, our model reduce the non-streaming FLOPS by 80\%.
Meanwhile, we achieve accuracy comparable or even slightly higher accuracy because we still keep the necessary attention layers, which can utilize the context information and achieve high accuracy.

Compared to full streaming encoders (CNN+RNN-T), our accuracy is much higher by 7\% in WER and 4.2\% in IC thanks to careful introduction of contextualization  
Meanwhile, our encoding latency is only higher by 0.012 - 0.016 RTF. 
Such an encoding difference will be diminished by the difference in decoding delays

\textbf{--- ABOVE --- }

%Concerning the encoding time, our system reduces it by 60\% compares to the conformer-m baseline and branchformer baseline.
%This reduction is attributed to the fact that the baseline local processing with the conformer model employs a transformer-based encoder and decoder, which requires complete data lengths to initiate processing. 

%By contrast, our system customizes the encoder structure, designing the initial layers (6/9) to exclusively comprise CNN-based modules. 
%\textbf{This modification enables the system to accommodate streaming data.}
%Figure ~\ref{fig:eval:fig-models} shows the breakdown of the encoder FLOPS of local baseline models. Compares to the branchformer and conformer models, our model has significantly fewer FLOPS. 
%Although the CNN+RNNT model is a fully streaming model, it compromises a lot on accuracy. Overall, our encoder  design represents the most feasible approach for balancing the trade-off between latency and accuracy.

%We compare the model specification shown in Table~\ref{tab:eval:models}. 
%Compares to the conformer-M model and the Branchformer model, our customized model encoder achieves similar or higher WER/IC with lower non-streaming latency and a comparable \xzlNote{comparable} model size. 
%\textbf{The late contextualization allows the encoder to start processing earlier with streaming data.} 
%In the table, we break down the encoder FLOPS into two part: the "embed" part and the "encoders" part. The "embed" part only contains CNN layers and an embed layer, naturally supports the streaming processing. 
%However, the "encoders" part in the baseline conformer and branchformer encoders include a transformer block in each layer, preventing it from starting processing before ingestion is finished.
%On the other hand, our late contextualized encoder only have 3 transformer layers at the end, make the 66\% computation can be finished in a streaming fashion. 
%Overall, the late contextualization help the \sys{} save 80\% encoding non-streaming FLOPS compare to the baseline models. \xzlNote{I don't understand the 80\% argument...(it shoudl be the streaming argument, instead of saving of flops)} \wrxNote{change to non-streaming FLOPS. need further discussion on encoder operation}
%The model RTF break down of each part shows in table~\ref{tab:eval:models2} is also consistent with the FLOPS result.

\input{tab-pilot}
%\paragraph{local path: Pilot decoding and decoding speedup}

\paragraph{Decoding speedup}

%\xzlNote{moved here and merge}
Moreover, our system reduces the decoding time by 50\% compares to all the local baselines.
This improvement is tied to the preliminary decoding outcomes from pilot decoding, which subsequently assist in the complete length decoding process and adaptively reduces the beam size, thus eliminating unnecessary computations.


Pilot decoding plays an important role in \sys{} local processing speed up. We conduct experiments to compare the pilot decoding's significance and its performance in different granularity. the result shows in table~\ref{tab:eval:pilot}. 
Pilot decoding with 1 second granularity can help decrease the RTF by 50\% when fully local processing compares to all the local baselines 
%This benefit could decrease \xzlNote{when cloud offloading increase}, \xzlNote{the logic is twisted. need straight up} 
Compares to offloading bases on perplexing score without pilot decoding and acceleration, The \sys{} still shows ~40\% RTF decrease on WER target 0.12, when 70\% of the data has been offload to cloud.


\xzlNote{talk about how granularity impact local path}
%it can improve, but with diminish return... a few sentences on why
Smaller granularity can further decrease the decoding RTF. As seen in table ~\ref{tab:eval:pilot} a granularity of 0.3s exhibits the lowest decoding RTF among all the granularity. This is because a smaller granularity can make the partial data of pilot decoding more similar to the full length data, thus yielding a more accurate preliminary decoding result and aiding in the reduction of the beam size during the full decoding process.


%\xzlNote{discuss the tradeoff... which hinges on...}
The hardware specification determines the boundary of the granularity. The granularity need to be larger than the longest execution time of pilot decoding. For board 1 with a weaker CPU, the best granularity is 1s. For board 2, the better CPU enables the 0.3s granularity choice.


\subsection{Efficacy of our offloading path}

\input{tab-offload}

\sys{} inspects the data and selectively offloads some of them to the cloud side. 
\textbf{Our offloading strategies effectively estimates the local processing confidence of the data and selects data with low confidence to the cloud, reducing the latency by 0.03 RTF as compared to sampling with pilot decoding speed up.}
\xzlNote{talk about target, nontarget...} \wrxNote{I talk about it in the later part when talk about pilot decoding granularity, as the table 5 doesn't have target nontarget data}
Moreover, we offload 10\%-15\% less data compare to sampling for reaching same accuracy targets. The experiment results are shown in Table~\ref{tab:eval:offload}.

We have experimented with several methods for estimating local processing confidence. 
First, we demonstrate that a popular prior approach, which involves adopting a BERT-style linear classifier for confidence estimation in transformer-based models, does not yield favorable results in SU tasks. 
This approach was previously employed in DeeBERT, where classification layers were trained for each BERT layer to estimate the confidence and decide whether to exit processing midway. %\xzlNote{cite and explain in detail}. 
However, this method proves ineffective for SU tasks, as the linear layer cannot be effectively trained with the available data, resulting in identical output estimations for all inputs. We assume it is equivalent to random offloading. 

Furthermore, we find three methods that have similar efficacy in estimating confidence: the CNN-based method, the LSTM based method and the perplexing score based method. 
The CNN approach employs a CNN model that takes the encoder's intermediate output as input, while the LSTM model uses features extracted from the pilot decoding beam search as input. The perplexing score is directly calculated from the pilot decoding result. As shown in the table, these three approaches yield similar RTF at different WER target. Compares to random offloading, they reduce the RTF by approximately 15\% . We choose the perplexing score based method for its low complexity.


\xzlNote{about we using pilot decoding for offloading decisions...}
Note that the LSTM method and the perplexing score method mentioned above are based on pilot decoding results, thus the pilot decoding granularity also has impact on selective offloading. From the table~\ref{tab:eval:pilot} we can see that as granularity becomes finer, the decoding results can better assist in  selective offloading. We define the data as target data if local WER larger than cloud WER. When the WER target is set to be 0.12, 0.3s granularity help the 
\xzlNote{target/non target should be introduced formally}
offloading target / non target ratio goes to 1.45, while 2s granularity have ratio 1.05. When WER target is 0.15, 0.3s target / non target ratio goes to 2.23, while 2s have ratio 1.43


\subsection{Sensitivity to system parameters} 
\xzlNote{can wait}
\paragraph{Hardware specification}
Better local hardware with more powerful CPU can help with decreasing overall RTF for different accuracy target. Figure~\ref{fig:eval:e2e} shows experiments conducted on Jetson Orin Nano and Odroid N2+. Odroid N2+ have better CPU performance, thus get lower RTF on all the accuracy targets. However, the pilot decoding speed up ratio maintains the same among different devices. Besides, better CPU enables faster local pilot inference, make the granularity possible to be more finegrained. 

\paragraph{Network latency}
Worse network condition and longer network latency makes \sys{} have more significant RTF decrease compare to random offload. 

==> recycle_buffer/intro_0731.tex <==
% !TeX root = main.tex

\section{Introduction}
\label{sec:intro}

Speech is a pervasive user interface. 
It is in particular useful to small embedded/IoT devices where hands free interactions are desirable. 
At the core of speech understanding are two ML tasks: 
transcribing the input to a textual sentence (e.g. ``xxxx''), 
called automatic speech recognition (ASR) \xzlNote{cite}; 
and further translating to a structured intent (e.g. ``yyyy''), 
called spoken language understanding (SLU) \xzlNote{cite}.
In this paper we refer both ASR and SLU as speech understanding (SU) tasks. 

Speech understanding has been challenging. 
Today, while narrated utterances (read after pre-defined text) can be transcribed or understood with high accuracy, 
utterances closer to human daily speeches still see a significant gap in accuracy \xzlNote{cite},
because of accents, lexical and grammar diversity, free-formed/irregular utterance, background noise...
%State-of-the-art (SOTA) 
Modern SU models typically embrace an encoder-decoder architecture \xzlNote{cite};
the decoder generates output tokens sequentially, called \textit{autoregression}. 
For instance, XXX has XXX parameters in XXXX transformer layers (XXX for encoding and YYY for decoding). 

To provide \su{} to embedded/IoT devices, 
the cloud and the devices offer complementary resources.
Cloud offers much richer compute resources as well as ease of model tuning and deployment. 
No wonder cloud execution is default to most commercial applications such as Google assistant and Amazon Alexa. \xzlNote{cite}
By comparison, 
on-device execution avoids network trips, which are vital to interactivity; 
it mitigates privacy concerns arising from 
the leak of speaker identity and sensitive entities and intents,
which are shown as real threats by recent work. \xzlNote{cite}
% the leak of speaker identity, biometrics; via speech transcripts -- semantics, sensitive entity, intents, etc. 

%\paragraph{Opportunity of early offload}
\paragraph{Design goal: a device/cloud cascade for SU}
Like many AI tasks \xzlNote{cite}, 
speech understanding would benefit from device/cloud collaborative executions. 
The device processes input utterances with a simple \su{} model, 
and only offloads the inputs of low confidence to the cloud which runs a big model. 
To further reduce overhead for the device, 
a key optimization is \textit{early offload}: 
the device makes offload decisions based on partial processing of an input. 
Early offload for speech is supported by workload studies \xzlNote{cite}:
most inputs are simple in acoustic variations and lexical structures, 
whereas fewer ones are rich and complex. 
The former inputs are likely resolved by the on-device model, 
while the latter inputs are worth the offload cost. 

%We apply a proven execution paradigm (cite vision/camera tasks..) -- early offload -- to speech understanding tasks. 

\paragraph{Challenges}
While device/cloud executions and early offloading are well understood for other perception (AI) tasks \xzlNote{cite}, 
they remain largely unexplored for SU. 
The nature of speech and SU models raises unique challenges. 

% While this goal is reminiscent of prior offloading engines (esp for vision/camera tasks), 
Not just a classification layer, but autoregressive sequence generation; 
beam search, hypothesis ranking and scoring, etc. 

streaming input / processing


\textbf{Model pipeline...}

early offload ... benefit is limited b/c it's latency bound

offload to the cloud has to wait for the ingestion to complete... when the last audio segment is there

so the network bandwidth is not a big deal


\textbf{Assessing confidence in autoregression}
To make offload decisions, 
the device needs to measure its confidence in (partial) processing results. 
This mechanism is called an \textit{offramp}. 
Prior work on early exit \xzlNote{cite} focused on classification tasks; 
%such as image classification; 
their offramps make tentative predictions, and the prediction entropy is used as the measure of confidence. 
This technique does not apply to SU:
(1) typically using an encoder-decoder architecture \xzlNote{cite}, 
the model generates output token by token, exploring multiple tentative sequences (called hypothesis) using complex beam search.
% in an autoregressive fashion \xzlNote{cite}. 
(2) the quality of final result is measured by XXX or word error rate (WER), not simply prediction accuracy. 
\wrxNote{(3) Generally speaking, prior research in the field has primarily focused on applying a simple classification layer to the intermediate representation of speech. However, this approach is insufficient in fully harnessing the underlying features, consequently leading to inaccurate estimations of the optimal strategy and offloading decisions in a local cloud collaboration scheme.}
% As we will show, the prediction entropy of individual token is a poor measure of the final outcome. 
As we will show, the per token entropy is a poor measure of the confidence. 
\wrxNote{As we will show, superfical feature like overall perplexing score is a poor measure of the confidence}

\textbf{Early exit based on incomplete inputs}
A unique aspect of SU is that the input (utterance) is streaming; 
the ingestion of an utterance takes seconds, comparable to the SU (inference) delay. 
Therefore, 
% it is beneficial to make early exit decisions \textit{before} the input is complete, 
% it is beneficial to make early exit \textit{before} the input is complete, 
it is beneficial to make early exit while the input is still being ingested, 
allowing the device extra time to prepare the input for offloading (See Section XXX for details). 
Existing early exit solutions do not apply here, as they decide based on partial processing of \textit{complete} inputs. \xzlNote{cite}
Furthermore, an encoder/decoder SU model expects an complete input in order to generate output tokens; 
it was unclear how/if it can assess confidence in output based on partial inputs. 


\paragraph{\sys{}}
To this end, we present a runtime system. 
Executing on a client device, \sys{} manages the execution of ASR/SLU tasks.
It has three notable designs.


% A new architecture of device/cloud cascade. 
\textbf{A new device/cloud pipeline (cascade?) for SU: }
The device runs a series of SU models; 
\wrxNote{a modular model with multiple choices for each module to accommodate different input and scenarios}
for efficiency, they share much of weights and computations
the first few ``early exit'' models attempt to output confidence and do not materialize output; 
\wrxNote{the first few exit points are off ramps that }
the later one is for both early exits and materializing output (in case of high confidence). 
A data sanitizing stage strips privacy information from data, if offload is decided. 
The whole cascade can be abstracted as a task graph. 


\textbf{Still useful:} restructure the encoder so it is (mostly) streaming; 
bottom layers convolution, a minimum number of top layers (attention) that require full input; 
\xzlNote{merge}
We customize a modern speech model (encoder-decoder, attention based): 
so that bottom layers (closer to input) execute convolution which only require partial inputs, 
attention computation (which require complete inputs) is pushed to the top layers (closer to output). 
By deferring the attention computation, the model can generate meaningful intermediate results as input is ingested; it does not lose the benefit of attention (contextualization). 
The intermediate (encoding) results can be used to decode offramps. 


\textbf{Novel offramps for autoregression...}
It is a miniature decoder (transformer) that consumes partial model execution on partial input; 
based on encoder-decoder scores and language model perplexity, 
it predicts the final confidence (if the on-device inference were to execute in full). 
We show how to train these offramps alongside the training of the on-device model. 
\textbf{Also:}
Partial inputs (short duration, inadequate information, incomplete beam search): hand crafted features, gradient boost, decision trees; 
Complete inputs (Bi-LSTM, sequence classification)

% We present a task scheduler (decision engine?)
\textbf{A scheduler for scheduling the cascade}: 
Question: which offramp to take; how to route inputs among local and cloud models?

Based on predictions made by offramps, 
the scheduler takes into account potential benefit (reduction in delays), potential accuracy gain, 
and routes the inputs among local models and the cloud. 
It orchestrates: 
local ingestion (streaming inputs); 
local encoding (multiple models, sharing?)
local offramps (tentative decoding, based on partial input)
local decoding (based on complete input)
offloading (data sanitizing/obfuscation), 




The scheduler abstracts the whole inference as a task graph, 
where nodes represent convolution, attention, off-ramps, and decoder; 
and edges capture data dependencies among nodes. 
The task scheduler starts from on-device execution path (inference), invokes offramps at various points, and judiciously switches to the offload path as it warrants. 
It makes scheduling decisions along two dimensions: input (should it consume more segments) and model layer (should it execute deeper layers). 
Furthermore, 
% it is resource conserving \xzlNote{cite}
it well utilizes resource for low delay: 
when encoding the streaming input cannot keep the device compute busy, 
the scheduler speculatively executes offload (sanitize tasks) even if it does not commit to offloading yet. 








\paragraph{Results}


\paragraph{Contributions}
We made three novel contributions. 

\begin{itemize}
\item An encoder-decoder model architecture (convolution on bottom layers; attention on top layers)
so that it suits early offloading on streaming (partial) inputs.

\item An off-ramp design (one-layer transformer) that predicts model confidence in generative output (autoregressive). Use a suite of optimizations: 
adaptive (?) beam width, language models, ...

\item A task scheduler: it judiciously inserts off-ramps into the task graph and switches from the on-device execution path to the offload path. 

\end{itemize}
	







 




==> recycle_buffer/motiv_0808.tex <==
\section{Motivations}
\label{sec:motiv}

\subsection{SU needs device/cloud executions}

\xzlNote{moved here, merge}
Today, while narrated utterances (read after pre-defined text) can be transcribed or understood with high accuracy, 
utterances closer to human daily speeches still see a significant gap in accuracy \xzlNote{cite},
because of accents, lexical and grammar diversity, free-formed/irregular utterance, background noise...
%State-of-the-art (SOTA) 

it also offers ease of model tuning and deployment. 


On-device execution alone still lags behind the SOTA accuracy (satisfactory experience) significantly.
(1) User expectation for SU keeps increasing, as reflected by benchmark advance. 
(2) SOTA models large and expensive, based on encoder-decoder, transformers, pretrained foundation models, etc. 
This entails warrants cloud offloading as needed (for certain inputs). 

No wonder cloud execution is default to most commercial applications such as Google assistant and Amazon Alexa. \xzlNote{cite}
% the leak of speaker identity, biometrics; via speech transcripts -- semantics, sensitive entity, intents, etc. 



\subsection{What's unique about speech}

\textbf{also a primer...}
Paradigm shifts from Markov models, to RNNs (neural network sequence modeling). 
Recent advance in SSL (attention-based models, encoder-decoder architecture) is another major breakthrough. 

\paragraph{Speech processing different from video processing}
Speech data has long ingestion time. State of the art transformer model requires the full length data. 

\paragraph{privacy through sanitizing}
Recent work shows that speech privacy risk can be mitigates via  preprocessing (sanitize) before offloading, 
which, again, incurs significant processing delays (3x of the input duration). 

\paragraph{offloading: latency bound...}

\subsection{Analysis of SLU overhead}

Breakdown: input, encoding, decoding, ...

For parallelism, encoding can be segment by segment. (Convolution, to extract local features)
Only the top layer is transformer. 

Encoding is less likely the limiting factor. 
It is much cheaper than decoding, which must emit each token (subword) sequentially. 

at ingestion time, 




\subsection{Early offload or early exit?}


\xzlNote{moved here. to merge}
This paper has a simple goal: combine the best of both worlds (per-input, dynamic decision between on-device execution and offloading). 
In the spirit of (early filters), an edge device can resolve simple inputs (by executing a local model) without offloading (lower delays; lower model capacity); 
offload more difficult inputs after sanitizing them (higher delays; large model capacity). 



Early exit: materialize results with sufficiently high confidence that the results are correct

\begin{itemize}
\item Only possible when input becomes complete
\item Need to run the (expensive) decoder
\end{itemize}
	

Early offload: send to the cloud with sufficiently low confidence (low scores) that the results are correct


Why early exit: 

\subsection{Speech processing: what is unique}
Speech processing is a general field with many different tasks related to speech signal. There are ASR, which focus on transcripting speech signals; SLU which goes further and extract the intent and entities in the speech. There are also TTS which generate Speech signal with existing transcripts, ST which directly translate the speech to other language, etc. In this  project we focus on ASR and SLU tasks, which are fundamental tasks in the speech, also usually become frontend of a large related system.

The speech signal exhibits a distinctive nature. The original dataset comprises a one-dimensional vector that represents a sampled recording of the voice signal. For instance, when utilizing a 16k sampling rate, the resulting vector will possess a length of 16k, corresponding to one second of voice data. In the context of Automatic Speech Recognition (ASR) and Spoken Language Understanding (SLU), the prevailing and widely accepted approach involves employing an encoder-decoder based model. The data undergoes an initial frontend processing step, wherein it is transformed into a frequency spectrum. Subsequently, the processed data traverses through a convolutional neural network (CNN) and transformer-based encoder to further extract essential features. Ultimately, the transformer-based decoder, supplemented by an optional language model, decodes the data in a token-by-token manner, frequently utilizing beam search to aid in the decoding process.

Speech processing, quite different from image processing, is still an unsolved problem on mobile device. Speech signal usually have a long ingestion time, while image processing always have a frame of image ready to be processed. The image processing usually adopt CNN based model. However, the speech processing need transformer based model to achieve state-of-the-art accuracy. Transformer based models rely on the attention mechanism and have relatively large parameter sizes. As a consequence, the speech processing systems usually need to wait until the data finish ingestion and locate the model on a cloud server. The cloud-device communication and data offloading raise a concern on privacy loss. 


\begin{itemize}
\item Streaming input
\item Contextualization is vital to accuracy
\item Autoregression with beam search
\end{itemize}

\subsection{Speech data (signal): complexity and chance}
Speech data exhibits complexity from various perspectives. Some example factors are environmental variations, sentence lexical structure (inverted sentences, clauses, etc.), specialized terms and entities, etc. Moreover, individual differences in speech habits, including accents, pitch, speed and other factors, compound the complexities reflected in all the aforementioned aspects.

Data with varying complexity could also be processed with different deep learning models. For instance, large cloud-based models generally exhibit higher overall accuracy in ASR/SLU tasks. However, a closer examination reveals that a substantial portion of relatively simple data achieves similar accuracy with both large and small models, whereas more challenging data shows considerable different processing outcomes. 

Given this diversity in data complexity and the corresponding model requirements, there is a pressing need to develop methods that enable precise model selection and offloading decisions. This optimization is essential to conserve computational resources and minimize potential privacy risks.

\subsection{Speech related model: state-of-the-art and their constraints}
The present state-of-the-art models in the field of speech processing, namely Wav2vec2, HuBERT, conformer, and branchformer, can be conceptually divided into three main components: the CNN feature extraction part (Encoder.embed), the encoder transformer/CNN stack part (Encoder.stack), and the decoder part. Although these previous models (Wav2vec2, HuBERT, conformer, branchformer) demonstrate reasonable accuracy, they typically possess large model sizes and rely on GPU support for efficient inference, make them less suitable for deployment on mobile devices. Furthermore, in the case of transformer-based encoders, the requirement for full-length data ingestion introduces execution delays as the system awaits data ingestion completion before initiating any model execution decision.

At the same time, we could see that in these transformer-based model, there exist a parameter redundancy issue. E.g. the branchformer paper mentioned that some transformer block in the encoder.stack part play a less important role. Following the direction, we design a model group that trying to overcome the parameter redundancy issue, also provide modules that works on partial streaming data.

==> recycle_buffer/motiv_0812.tex <==
\section{Motivations}
\label{sec:motiv}

\subsection{SU needs device/cloud executions}

\xzlNote{moved here, merge}
Today, while narrated utterances (read after pre-defined text) can be transcribed or understood with high accuracy, 
utterances closer to human daily speeches still see a significant gap in accuracy \xzlNote{cite},
because of accents, lexical and grammar diversity, free-formed/irregular utterance, background noise...
%State-of-the-art (SOTA) 

it also offers ease of model tuning and deployment. 


On-device execution alone still lags behind the SOTA accuracy (satisfactory experience) significantly.
(1) User expectation for SU keeps increasing, as reflected by benchmark advance. 
(2) SOTA models large and expensive, based on encoder-decoder, transformers, pretrained foundation models, etc. 
This entails warrants cloud offloading as needed (for certain inputs). 

No wonder cloud execution is default to most commercial applications such as Google assistant and Amazon Alexa. \xzlNote{cite}
% the leak of speaker identity, biometrics; via speech transcripts -- semantics, sensitive entity, intents, etc. 



\subsection{What's unique about speech}

\textbf{also a primer...}
Paradigm shifts from Markov models, to RNNs (neural network sequence modeling). 
Recent advance in SSL (attention-based models, encoder-decoder architecture) is another major breakthrough. 

\paragraph{Speech processing different from video processing}
Speech data has long ingestion time. State of the art transformer model requires the full length data. 

\paragraph{privacy through sanitizing}
Recent work shows that speech privacy risk can be mitigates via  preprocessing (sanitize) before offloading, 
which, again, incurs significant processing delays (3x of the input duration). 

\paragraph{offloading: latency bound...}

\subsection{Analysis of SLU overhead}

Breakdown: input, encoding, decoding, ...

For parallelism, encoding can be segment by segment. (Convolution, to extract local features)
Only the top layer is transformer. 

Encoding is less likely the limiting factor. 
It is much cheaper than decoding, which must emit each token (subword) sequentially. 

at ingestion time, 




\subsection{Early offload or early exit?}


\xzlNote{moved here. to merge}
This paper has a simple goal: combine the best of both worlds (per-input, dynamic decision between on-device execution and offloading). 
In the spirit of (early filters), an edge device can resolve simple inputs (by executing a local model) without offloading (lower delays; lower model capacity); 
offload more difficult inputs after sanitizing them (higher delays; large model capacity). 



Early exit: materialize results with sufficiently high confidence that the results are correct

\begin{itemize}
\item Only possible when input becomes complete
\item Need to run the (expensive) decoder
\end{itemize}
	

Early offload: send to the cloud with sufficiently low confidence (low scores) that the results are correct


Why early exit: 

\subsection{Speech processing: what is unique}
Speech processing is a general field with many different tasks related to speech signal. There are ASR, which focus on transcripting speech signals; SLU which goes further and extract the intent and entities in the speech. There are also TTS which generate Speech signal with existing transcripts, ST which directly translate the speech to other language, etc. In this  project we focus on ASR and SLU tasks, which are fundamental tasks in the speech, also usually become frontend of a large related system.

The speech signal exhibits a distinctive nature. The original dataset comprises a one-dimensional vector that represents a sampled recording of the voice signal. For instance, when utilizing a 16k sampling rate, the resulting vector will possess a length of 16k, corresponding to one second of voice data. In the context of Automatic Speech Recognition (ASR) and Spoken Language Understanding (SLU), the prevailing and widely accepted approach involves employing an encoder-decoder based model. The data undergoes an initial frontend processing step, wherein it is transformed into a frequency spectrum. Subsequently, the processed data traverses through a convolutional neural network (CNN) and transformer-based encoder to further extract essential features. Ultimately, the transformer-based decoder, supplemented by an optional language model, decodes the data in a token-by-token manner, frequently utilizing beam search to aid in the decoding process.

Speech processing, quite different from image processing, is still an unsolved problem on mobile device. Speech signal usually have a long ingestion time, while image processing always have a frame of image ready to be processed. The image processing usually adopt CNN based model. However, the speech processing need transformer based model to achieve state-of-the-art accuracy. Transformer based models rely on the attention mechanism and have relatively large parameter sizes. As a consequence, the speech processing systems usually need to wait until the data finish ingestion and locate the model on a cloud server. The cloud-device communication and data offloading raise a concern on privacy loss. 


\begin{itemize}
\item Streaming input
\item Contextualization is vital to accuracy
\item Autoregression with beam search
\end{itemize}

\subsection{Speech data (signal): complexity and chance}
Speech data exhibits complexity from various perspectives. Some example factors are environmental variations, sentence lexical structure (inverted sentences, clauses, etc.), specialized terms and entities, etc. Moreover, individual differences in speech habits, including accents, pitch, speed and other factors, compound the complexities reflected in all the aforementioned aspects.

Data with varying complexity could also be processed with different deep learning models. For instance, large cloud-based models generally exhibit higher overall accuracy in ASR/SLU tasks. However, a closer examination reveals that a substantial portion of relatively simple data achieves similar accuracy with both large and small models, whereas more challenging data shows considerable different processing outcomes. 

Given this diversity in data complexity and the corresponding model requirements, there is a pressing need to develop methods that enable precise model selection and offloading decisions. This optimization is essential to conserve computational resources and minimize potential privacy risks.

\subsection{Speech related model: state-of-the-art and their constraints}
The present state-of-the-art models in the field of speech processing, namely Wav2vec2, HuBERT, conformer, and branchformer, can be conceptually divided into three main components: the CNN feature extraction part (Encoder.embed), the encoder transformer/CNN stack part (Encoder.stack), and the decoder part. Although these previous models (Wav2vec2, HuBERT, conformer, branchformer) demonstrate reasonable accuracy, they typically possess large model sizes and rely on GPU support for efficient inference, make them less suitable for deployment on mobile devices. Furthermore, in the case of transformer-based encoders, the requirement for full-length data ingestion introduces execution delays as the system awaits data ingestion completion before initiating any model execution decision.

At the same time, we could see that in these transformer-based model, there exist a parameter redundancy issue. E.g. the branchformer paper mentioned that some transformer block in the encoder.stack part play a less important role. Following the direction, we design a model group that trying to overcome the parameter redundancy issue, also provide modules that works on partial streaming data.

==> scripts/Makefile <==
# batch convert all .pptx files in a directory to .pdf  
# files and crop them. 
# 
# to be used in conjunction with ppt.vbs, which converts
# a .pptx file into a pdf. 
#
# usage: copy this file and ppt.vbs to figs/ and run make
# there
#
# environment: win 10 cmd
#

docobjects := $(patsubst %.docx,%.pdf,$(wildcard *.docx)) $(patsubst %.dox,%.pdf,$(wildcard *.dox))
pptobjects := $(patsubst %.pptx,%.pdf,$(wildcard *.pptx))

current_dir  := $(shell cd)

all : check_overlap $(docobjects) $(pptobjects) 

	
docx : $(docobjects)

pptx : $(pptobjects)

clean :
	del /Q $(docobjects) $(pptobjects)

check_overlap :
	@echo "$(current_dir)"
		
		
%.pdf.uncrop : %.docx
	"c:\Windows\SysWOW64\cscript.exe" "$(scriptDir)\docx.vbs" "$(current_dir)\$^" "$(current_dir)\$@"

%.pdf.uncrop : %.dox
	"c:\Windows\SysWOW64\cscript.exe" "$(scriptDir)\docx.vbs" "$(current_dir)\$^" "$(current_dir)\$@"

%.pdf.uncrop : %.pptx
	"c:\Windows\SysWOW64\cscript.exe" "$(scriptDir)\ppt.vbs" "$(current_dir)\$^" "$(current_dir)\$@"

%.pdf: %.pdf.uncrop
	"$(scriptDir)\bin\pdfcrop.exe" $^ $@
	
	
.PHONY: check_overlap all docx pptx

==> scripts/bin/pdfcrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__


==> summary__Felix_s_conflicted_copy_2023-11-30_.tex <==
% !TeX root = main.tex
\section{Conclusions}
We present \sys{}, a novel system for fast speech processing in SU tasks. \sys{} contributes late contextualization, beam collapse/ termination, and CTC leap for local execution; 
and confidence estimation for selective offloading. 
%The former allows \sys{} accelerate local execution while the latter one enables users to better trade-off the accuracy and latency. 
All optimizations combined, \sys{} speeds up its local path by 2x and reduces the offloading needs by 2x in its offloading path.



%We present \sys{}, a novel system for fast speech processing in SU tasks. \sys{} contributes late contextualization, beam collapse, beam search early termination and ctc leap techniques for local execution and confidence estimation techniques for hybrid execution collaborating with cloud service. The former allows \sys{} accelerate local execution while the latter one enables users to better trade-off the accuracy and latency. With the techniques, the \sys{} can reduce 2x for local execution, and reduce 50\% or more offloading and cloud service queries for hybrid execution. 

==> tab-modelrtf.tex <==
% !TeX root = main.tex
\begin{table}[t]
    \centering
        \includegraphics[width=0.48\textwidth{}]{./figs/modelrtf}
        \caption{Our local execution path incur lower latencies (reported as RTF) for both encoding and decoding,  as compared to other on-device models. The decoding RTF with different speedup setting is also shown. LP: length prediction, BR: beam reduce, CS: ctc prefix scoring speedup}
        \label{tab:modelrtf}        
\end{table}

% while retaining strong accuracy. Our model minimize the non streaming RTF while keep high accuracy. 
% \textit{OnDevice} models.

